Measurement of the W Boson Polarization in Top Decay at CDF at s**(1/2) = 1.8 TeV

The polarization of the $W$ boson in $t \to W b$ decay is unambiguously predicted by the Standard Model of weak interactions and is a powerful test of our understanding of the $tbW$ vertex. The subsequent $W \to l \nu$ decay serves as a polarimeter for the $W$, and the invariant mass of the lepton and $b$ quark in top decay provides a measurement of the $W$ decay angle. In this paper we present a measurement of the decay rate of the W produced from the decay of the top quark in the hypothesis of V+A structure of the tWb vertex. We find no evidence for the non-standard V+A vertex and set a limit on $f_{V+A}$ $<$ 0.80 @ 95% confidence level. By combining this result with a complementary observable in the same data, we assign a limit of $f_{V+A}$ $<$ 0.61 @ 95% CL.

==> author.tex <==
%auto-ignore
\author{
D. Acosta $^{14}$, T. Affolder $^{25}$, H. Akimoto $^{50}$,
M. G. Albrow $^{13}$, D. Ambrose $^{37}$, D. Amidei $^{28}$, K. Anikeev
$^{27}$, J. Antos $^{1}$, G. Apollinari $^{13}$, T. Arisawa $^{50}$,
A. Artikov $^{11}$, T. Asakawa $^{48}$, W. Ashmanskas $^{10}$, F. Azfar
$^{35}$, P. Azzi-Bacchetta $^{36}$, N. Bacchetta $^{36}$, H. Bachacou
$^{25}$, W. Badgett $^{13}$, S. Bailey $^{18}$, P. de Barbaro $^{41}$,
A. Barbaro-Galtieri $^{25}$, V. E. Barnes $^{40}$, B. A. Barnett $^{21}$,
S. Baroiant $^{5}$, M. Barone $^{15}$, G. Bauer $^{27}$, F. Bedeschi $^{38}$,
S. Behari $^{21}$, S. Belforte $^{47}$, W. H. Bell $^{17}$, G. Bellettini
$^{38}$, J. Bellinger $^{51}$, D. Benjamin $^{12}$, J. Bensinger $^{4}$,
A. Beretvas $^{13}$, J. Berryhill $^{10}$, A. Bhatti $^{42}$, M. Binkley
$^{13}$, D. Bisello $^{36}$, M. Bishai $^{13}$, R. E. Blair $^{2}$,
C. Blocker $^{4}$, K. Bloom $^{28}$, B. Blumenfeld $^{21}$, S. R. Blusk
$^{41}$, A. Bocci $^{42}$, A. Bodek $^{41}$, G. Bolla $^{40}$, A. Bolshov
$^{27}$, Y. Bonushkin $^{6}$, D. Bortoletto $^{40}$, J. Boudreau $^{39}$,
A. Brandl $^{31}$, C. Bromberg $^{29}$, M. Brozovic $^{12}$, E. Brubaker
$^{25}$, N. Bruner $^{31}$, J. Budagov $^{11}$, H. S. Budd $^{41}$,
K. Burkett $^{18}$, G. Busetto $^{36}$, K. L. Byrum $^{2}$, S. Cabrera
$^{12}$, P. Calafiura $^{25}$, M. Campbell $^{28}$, W. Carithers $^{25}$,
J. Carlson $^{28}$, D. Carlsmith $^{51}$, W. Caskey $^{5}$, A. Castro $^{3}$,
D. Cauz $^{47}$, A. Cerri $^{38}$, L. Cerrito $^{20}$, A. W. Chan $^{1}$,
P. S. Chang $^{1}$, P. T. Chang $^{1}$, J. Chapman $^{28}$, C. Chen $^{37}$,
Y. C. Chen $^{1}$, M.-T. Cheng $^{1}$, M. Chertok $^{5}$, G. Chiarelli
$^{38}$, I. Chirikov-Zorin $^{11}$, G. Chlachidze $^{11}$, F. Chlebana
$^{13}$, L. Christofek $^{20}$, M. L. Chu $^{1}$, J. Y. Chung $^{33}$,
W.-H. Chung $^{51}$, Y. S. Chung $^{41}$, C. I. Ciobanu $^{33}$, A. G. Clark
$^{16}$, M. Coca $^{38}$, A. P. Colijn $^{13}$, A. Connolly $^{25}$,
M. Convery $^{42}$, J. Conway $^{43}$, M. Cordelli $^{15}$, J. Cranshaw
$^{45}$, R. Culbertson $^{13}$, D. Dagenhart $^{4}$, S. D'Auria $^{17}$,
S. De Cecco $^{43}$, F. DeJongh $^{13}$, S. Dell'Agnello $^{15}$,
M. Dell'Orso $^{38}$, S. Demers $^{41}$, L. Demortier $^{42}$, M. Deninno
$^{3}$, D. De Pedis $^{43}$, P. F. Derwent $^{13}$, T. Devlin $^{43}$,
C. Dionisi $^{43}$, J. R. Dittmann $^{13}$, A. Dominguez $^{25}$, S. Donati
$^{38}$, M. D'Onofrio $^{38}$, T. Dorigo $^{36}$, I. Dunietz $^{13}$, N. Eddy
$^{20}$, K. Einsweiler $^{25}$, E. Engels Jr. $^{39}$, R. Erbacher
$^{13}$, D. Errede $^{20}$, S. Errede $^{20}$, R. Eusebi $^{41}$, Q. Fan
$^{41}$, H.-C. Fang $^{25}$, S. Farrington $^{17}$, R. G. Feild $^{52}$,
J. P. Fernandez $^{40}$, C. Ferretti $^{38}$, R. D. Field $^{14}$, I. Fiori
$^{3}$, B. Flaugher $^{13}$, L. R. Flores-Castillo $^{39}$, G. W. Foster
$^{13}$, M. Franklin $^{18}$, J. Freeman $^{13}$, J. Friedman $^{27}$,
Y. Fukui $^{23}$, I. Furic $^{27}$, S. Galeotti $^{38}$, A. Gallas $^{32}$,
M. Gallinaro $^{42}$, T. Gao $^{37}$, M. Garcia-Sciveres $^{25}$,
A. F. Garfinkel $^{40}$, P. Gatti $^{36}$, C. Gay $^{52}$, D. W. Gerdes
$^{28}$, E. Gerstein $^{9}$, S. Giagu $^{43}$, P. Giannetti $^{38}$, K. Giolo
$^{40}$, M. Giordani $^{5}$, P. Giromini $^{15}$, V. Glagolev $^{11}$,
D. Glenzinski $^{13}$, M. Gold $^{31}$, J. Goldstein $^{13}$, G. Gomez
$^{8}$, M. Goncharov $^{44}$, I. Gorelov $^{31}$, A. T. Goshaw $^{12}$,
Y. Gotra $^{39}$, K. Goulianos $^{42}$, C. Green $^{40}$, A. Gresele $^{36}$,
G. Grim $^{5}$, C. Grosso-Pilcher $^{10}$, M. Gu enther $^{40}$, G. Guillian
$^{28}$, J. Guimaraes da Costa $^{18}$, R. M. Haas $^{14}$, C. Haber $^{25}$,
S. R. Hahn $^{13}$, E. Halkiadakis $^{41}$, C. Hall $^{18}$, T. Handa
$^{19}$, R. Ha ndler $^{51}$, F. Happacher $^{15}$, K. Hara $^{48}$,
A. D. Hardman $^{40}$, R. M. Harris $^{13}$, F. Hartmann $^{22}$,
K. Hatakeyama $^{42}$, J. Hauser $^{6}$, J. Heinrich $^{37}$, A. Heiss
$^{22}$, M. Hennecke $^{22}$, M. Herndon $^{21}$, C. Hill $^{7}$, A. Hocker
$^{41}$, K. D. Hoffman $^{10}$, R. Hollebeek $^{37}$, L. Holloway $^{20}$,
S. Hou $^{1}$, B. T. Huffman $^{35}$, R. Hughes $^{33}$, J. Huston $^{29}$,
J. Huth $^{18}$, H. Ikeda $^{48}$, J. Incandela $^{7}$, G. Introzzi $^{38}$,
M. Iori $^{43}$,A. Ivanov $^{41}$, J. Iwai $^{50}$, Y. Iwata $^{19}$,
B. Iyutin $^{27}$, E. James $^{28}$, M. Jones $^{37}$, U. Joshi $^{13}$,
H. Kambara $^{16}$, T. Kamon $^{44}$, T. Kaneko $^{48}$, M. Karagoz Unel
$^{32}$, K. Karr $^{49}$, S. Kartal $^{13}$, H. Kasha $^{52}$, Y. Kato
$^{34}$, T. A. Keaffaber $^{40}$, K. Kelley $^{27}$, M. Kelly $^{28}$,
R. D. Kennedy $^{13}$, R. Kephart $^{13}$, D. Khazins $^{12}$, T. Kikuchi
$^{48}$, B. Kilminster $^{41}$, B. J. Kim $^{24}$, D. H. Kim $^{24}$,
H. S. Kim $^{20}$, M. J. Kim $^{9}$, S. B. Kim $^{24}$, S. H. Kim $^{48}$,
T. H. Kim $^{27}$, Y. K. Kim $^{25}$, M. Kirby $^{12}$, M. Kirk $^{4}$,
L. Kirsch $^{4}$, S. Klimenko $^{14}$, P. Koehn $^{33}$, K. Kondo $^{50}$,
J. Konigsberg $^{14}$, A. Korn $^{27}$, A. Korytov $^{14}$, K. Kotelnikov
$^{30}$, E. Kovacs $^{2}$, J. Kroll $^{37}$, M. Kruse $^{12}$, V. Krutelyov
$^{44}$, S. E. Kuhlmann $^{2}$, K. Kurino $^{19}$, T. Kuwabara $^{48}$,
A. T. Laasanen $^{40}$, N. Lai $^{10}$, S. Lami $^{42}$, S. Lammel $^{13}$,
J. Lancaster $^{12}$, K. Lannon $^{20}$, M. Lancaster $^{26}$, R. Lander
$^{5}$, A. Lath $^{43}$, G. Latino $^{31}$, T. LeCompte $^{2}$, Y. Le
$^{21}$, S. W. Lee $^{44}$, N. Leonardo $^{27}$, S. Leone $^{38}$,
J. D. Lewis $^{13}$, K. Li $^{53}$, M. Lindgren $^{6}$, T. M. Liss $^{20}$,
J. B. Liu $^{41}$, T. Liu $^{13}$, Y. C. Liu $^{1}$, D. O. Litvintsev
$^{13}$, O. Lobban $^{45}$, N. S. Lockyer $^{37}$, A. Loginov $^{30}$,
J. Loken $^{35}$, M. Loreti $^{36}$, D. L ucchesi $^{36}$, P. Lukens $^{13}$,
S. Lusin $^{51}$, L. Lyons $^{35}$, J. Lys $^{25}$, R. Madrak $^{18}$,
K. Maeshima $^{13}$, P. Maksimovic $^{21}$, L. Malferrari $^{3}$, M. Mangano
$^{38}$, G. Manca $^{35}$, M. Mariotti $^{36}$, G. Martignon $^{36}$,
M. Martin $^{21}$, A. Martin $^{52}$, V. Martin $^{32}$, J. A. J. Matthews
$^{31}$, P. Mazzanti $^{3}$, K. S. McFarland $^{41}$, P. McIntyre $^{44}$,
M. Menguzzato $^{36}$, A. Menzione $^{38}$, P. Merkel $^{13}$, C. Mesropian
$^{42}$, A. Meyer $^{13}$, T. Miao $^{13}$, R. Miller $^{29}$, J. S. Miller
$^{28}$, H. Minato $^{48}$, S. Miscetti $^{15}$, M. Mishina $^{23}$,
G. Mitselmakher $^{14}$, Y. Miyazaki $^{34}$, N. Moggi $^{3}$, E. Moore
$^{31}$, R. Moore $^{28}$, Y. Morita $^{23}$, T. Moulik $^{40}$, M. Mulhearn
$^{27}$, A. Mukherjee $^{13}$, T. Muller $^{22}$, A. Munar $^{38}$, P. Murat
$^{13}$, S. Murgia $^{29}$, J. Nachtman $^{6}$, V. Nagaslaev $^{45}$, S. Nahn
$^{52}$, H. Nakada $^{48}$, I. Nakano $^{19}$, R. Napora $^{21}$, C. Nelson
$^{13}$, T. Nelson $^{13}$, C. Neu $^{33}$, M. S. Neubauer $^{27}$,
D. Neuberger $^{22}$, C. Newman-Holmes $^{13}$, C.-Y. P. Ngan $^{27}$,
T. Nigmanov $^{39}$, H. Niu $^{4}$, L. Nodulman $^{2}$, A. Nomerotski
$^{14}$, S. H. Oh $^{12}$, Y. D. Oh $^{24}$, T. Ohmoto $^{19}$, T. Ohsugi
$^{19}$, R. Oishi $^{48}$, T. Okusawa $^{34}$, J. Olsen $^{51}$, W. Orejudos
$^{25}$, C. Pagliarone $^{38}$, F. Palmonari $^{38}$, R. Paoletti $^{38}$,
V. Papadimitriou $^{45}$, D. Partos $^{4}$, J. Patrick $^{13}$, G. Pauletta
$^{47}$, M. Paulini $^{9}$, T. Pauly $^{35}$, C. Paus $^{27}$, D. Pellett
$^{5}$, A. Penzo $^{47}$, L. Pescara $^{36}$, T. J. Phillips $^{12}$, G. Pi
acentino $^{38}$, J. Piedra $^{8}$, K. T. Pitts $^{20}$, A. Pompos $^{40}$,
L. Pondrom $^{51}$, G. Pope $^{39}$, T. Pratt $^{35}$, F. Prokoshin $^{11}$,
J. Proudfoot $^{2}$, F. Ptohos $^{15}$, O. Pukhov $^{11}$, G. Punzi $^{38}$,
J. Rademacker $^{35}$, A. Rakitine $^{27}$, F. Ratnikov $^{43}$, D. Reher
$^{25}$, A. Reichold $^{35}$, P. Renton $^{35}$, M. Rescigno $^{43}$,
A. Ribon $^{36}$, W. Riegler $^{18}$, F. Rimondi $^{3}$, L. Ristori $^{38}$,
M. Riveline $^{46}$, W. J. Robertson $^{12}$, T. Rodrigo $^{8}$, S. Rolli
$^{49}$, L. Rosenson $^{27}$, R. Roser $^{13}$, R. Rossin $^{36}$, C. Rott
$^{40}$, A. Roy $^{40}$, A. Ruiz $^{8}$, D. Ryan $^{49}$, A. Safonov $^{5}$,
R. St. Denis $^{17}$, W. K. Sakumoto $^{41}$, D. Saltzberg $^{6}$, C. Sanchez
$^{33}$, A. Sansoni $^{15}$, L. Santi $^{47}$, S. Sarkar $^{43}$, H. Sato
$^{48}$, P. Savard $^{46}$, A. Savoy-Navarro $^{13}$, P. Schlabach $^{13}$,
E. E. Schmidt $^{13}$, M. P. Schmidt $^{52}$, M. Schmitt $^{32}$,
L. Scodellaro $^{36}$, A. Scott $^{6}$, A. Scribano $^{38}$, A. Sedov
$^{40}$, S. Seidel $^{31}$, Y. Seiya $^{48}$, A. Semenov $^{11}$, F. Semeria
$^{3}$, T. Shah $^{27}$, M. D. Shapiro $^{25}$, P. F. Shepard $^{39}$,
T. Shibayama $^{48}$, M. Shimojima $^{48}$, M. Shochet $^{10}$, A. Sidoti
$^{36}$, J. Siegrist $^{25}$, A. Sill $^{45}$, P. Sinervo $^{46}$, P. Singh
$^{20}$, A. J. Slaughter $^{52}$, K. Sliwa $^{49}$, F. D. Snider $^{13}$,
R. Snihur $^{26}$, A. Solodsky $^{42}$, J. Spalding $^{13}$, T . Speer
$^{16}$, M. Spezziga $^{45}$, P. Sphicas $^{27}$, F. Spinella $^{38}$,
M. Spiropulu $^{10}$, L. Spiegel $^{13}$, J. Steele $^{51}$, A. Stefanini
$^{38}$, J. Strologas $^{20}$, F. Strumia $^{16}$, D. Stuart $^{7}$,
A. Sukhanov $^{14}$, K. Sumorok $^{27}$, T. Suzuki $^{48}$, T. Takano
$^{35}$, R. Takashima $^{19}$, K. Takikawa $^{48}$, P. Tamburello $^{12}$,
M. Tanaka $^{48}$, B. Tannenbaum $^{6}$, M. Tecchio $^{28}$, R. J. Tesarek
$^{13}$, P. K. Teng $^{1}$, K. Terashi $^{42}$, S. Tether $^{27}$,
A. S. Thompson $^{17}$, E. Thomson $^{33}$, R. Thurman-Keup $^{2}$, P. Tipton
$^{41}$, S. Tkaczyk $^{13}$, D. Toback $^{44}$, K. Tollefson $^{29}$,
A. Tollestrup $^{13}$, D. Tonelli $^{38}$, M. Tonnesmann $^{29}$, H. Toyoda
$^{34}$, W. Trischuk $^{46}$, J. F. de Troconiz $^{18}$, J. Tseng $^{27}$,
D. Tsybychev $^{14}$, N. Turini $^{38}$, F. Ukegawa $^{48}$, T. Unverhau
$^{17}$, T. Vaiciulis $^{41}$, J. Valls $^{43}$, E. Vataga $^{38}$, S. Vejcik
III $^{13}$, G. Velev $^{13}$, G. Veramendi $^{25}$, R. Vidal $^{13}$,
I. Vila $^{8}$, R. Vilar $^{8}$, I. Volobouev $^{25}$, M. von der Mey $^{6}$,
D. Vucinic $^{27}$, R. G. Wagner $^{2}$, R. L. Wagner $^{13}$, W. Wagner
$^{22}$, N. B. Wallace $^{43}$, Z. Wan $^{43}$, C. Wang $^{12}$, M. J. Wang
$^{1}$, S. M. Wang $^{14}$, B. Ward $^{17}$, S. Waschke $^{17}$, T. Watanabe
$^{48}$, D. Waters $^{26}$, T. Watts $^{43}$, M. Weber $^{25}$, H. Wenzel
$^{22}$, W. C. Wester III $^{13}$, B. Whitehouse $^{49}$, A. B. Wicklund
$^{2}$, E. Wicklund $^{13}$, T. Wilkes $^{5}$, H. H. Williams $^{37}$,
P. Wilson $^{13}$, B. L. Winer $^{33}$, D. Winn $^{28}$, S. Wolbers $^{13}$,
D. Wolinski $^{28}$, J. Wolinski $^{29}$, S. Wolinski $^{28}$, M. Wolter
$^{49}$, S. Worm $^{43}$, X. Wu $^{16}$, F. W\"urthwein $^{27}$, J. Wyss
$^{38}$, U. K. Yang $^{10}$, W. Yao $^{25}$, G. P. Yeh $^{13}$, P. Yeh
$^{1}$, K. Yi $^{21}$, J. Yoh $^{13}$, C. Yosef $^{29}$, T. Yoshida $^{34}$,
I. Yu $^{24}$, S. Yu $^{37}$, Z. Yu $^{52}$, J. C. Yun $^{13}$, L. Zanello
$^{43}$, A. Zanetti $^{47}$, F. Zetti $^{25}$, and S. Zucchelli $^{3}$
}

\affiliation{
   {\eightit Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic
of China } \\
   $^{2}$ {\eightit Argonne National Laboratory, Argonne, Illinois 60439  } \\
   $^{3}$ {\eightit Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127
Bologna, Italy } \\
   $^{4}$ {\eightit Brandeis University, Waltham, Massachusetts 02254 } \\
   $^{5}$ {\eightit University of California at Davis, Davis, California 95616 } \\
   $^{6}$ {\eightit University of California at Los Angeles, Los Angeles, California 90024 } \\ 
   $^{7}$ {\eightit University of California at Santa Barbara, Santa Barbara, California 93106  } \\
   $^{8}$ {\eightit Instituto de Fisica de Cantabria, CSIC-University of Cantabria,
39005 Santander, Spain  } \\
   $^{9}$ {\eightit Carnegie Mellon University, Pittsburgh, PA 15218  } \\
  $^{10}$ {\eightit Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637  } \\
  $^{11}$ {\eightit Joint Institute for Nuclear Research, RU-141980 Dubna, Russia  } \\
  $^{12}$ {\eightit Duke University, Durham, North Carolina 27708  } \\
  $^{13}$ {\eightit Fermi National Accelerator Laboratory, Batavia, Illinois 60510  } \\
  $^{14}$ {\eightit University of Florida, Gainesville, Florida 32611  } \\
  $^{15}$ {\eightit Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica
Nucleare, I-00044 Frascati, Italy  } \\
  $^{16}$ {\eightit University of Geneva, CH-1211 Geneva 4, Switzerland  } \\
  $^{17}$ {\eightit Glasgow University, Glasgow G12 8QQ, United Kingdom  } \\
  $^{18}$ {\eightit Harvard University, Cambridge, Massachusetts 02138  } \\
  $^{19}$ {\eightit Hiroshima University, Higashi-Hiroshima 724, Japan  } \\
  $^{20}$ {\eightit University of Illinois, Urbana, Illinois 61801  } \\
  $^{21}$ {\eightit The Johns Hopkins University, Baltimore, Maryland 21218  } \\
  $^{22}$ {\eightit Institut für Experimentelle Kernphysik, Universität Karlsruhe,
76128 Karlsruhe, Germany  } \\
  $^{23}$ {\eightit Center for High Energy Physics: Kyungpook National University,
Taegu 702-701; Seoul National University, Seoul 151-742; and SungKyunKwan
University, Suwon 440-746; Korea  } \\
  $^{24}$ {\eightit High Energy Accelerator Research Organization (KEK), Tsukuba,
Ibaraki 305, Japan  } \\
  $^{25}$ {\eightit Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley,
California 94720  } \\
  $^{26}$ {\eightit University College London, London WC1E 6BT, United Kingdom  } \\
  $^{27}$ {\eightit Massachusetts Institute of Technology, Cambridge, Massachusetts
02139  } \\
  $^{28}$ {\eightit University of Michigan, Ann Arbor, Michigan 48109  } \\
  $^{29}$ {\eightit Michigan State University, East Lansing, Michigan 48824  } \\
  $^{30}$ {\eightit Institution for Theoretical and Experimental Physics, ITEP,,
Moscow 117259, Russia  } \\
  $^{31}$ {\eightit University of New Mexico, Albuquerque, New Mexico 87131  } \\
  $^{32}$ {\eightit Northwestern University, Evanston, Illinois 60208  } \\
  $^{33}$ {\eightit The Ohio State University, Columbus, Ohio 43210  } \\
  $^{34}$ {\eightit Osaka City University, Osaka 588, Japan  } \\
  $^{35}$ {\eightit University of Oxford, Oxford OX1 3RH, United Kingdom  } \\
  $^{36}$ {\eightit Universita di Padova, Istituto Nazionale di Fisica Nucleare,
Sezione di Padova, I-35131 Padova, Italy  } \\
  $^{37}$ {\eightit University of Pennsylvania, Philadelphia, Pennsylvania 19104  } \\
  $^{38}$ {\eightit Istituto Nazionale di Fisica Nucleare, University and Scuola
Normale Superiore of Pisa, I-56100 Pisa, Italy  } \\
  $^{39}$ {\eightit University of Pittsburgh, Pittsburgh, Pennsylvania 15260  } \\
  $^{40}$ {\eightit Purdue University, West Lafayette, Indiana 47907  } \\
  $^{41}$ {\eightit University of Rochester, Rochester, New York 14627  } \\
  $^{42}$ {\eightit Rockefeller University, New York, New York 10021  } \\
  $^{43}$ {\eightit Instituto Nazionale de Fisica Nucleare, Sezione di Roma, University di Roma I, "La Sapienza," I-00185 Roma, Italy  } \\
  $^{44}$ {\eightit Rutgers University, Piscataway, New Jersey 08855  } \\
  $^{45}$ {\eightit Texas A\&M University, College Station, Texas 77843  } \\
  $^{46}$ {\eightit Texas Tech University, Lubbock, Texas 79409  } \\
  $^{47}$ {\eightit Institute of Particle Physics, University of Toronto, Toronto
M5S 1A7, Canada  } \\
  $^{48}$ {\eightit Istituto Nazionale di Fisica Nucleare, University of
Trieste/Udine, Italy  } \\
  $^{49}$ {\eightit University of Tsukuba, Tsukuba, Ibaraki 305, Japan  } \\
  $^{50}$ {\eightit Tufts University, Medford, Massachusetts 02155  } \\
  $^{51}$ {\eightit Waseda University, Tokyo 169, Japan  } \\
  $^{52}$ {\eightit University of Wisconsin, Madison, Wisconsin 53706  } \\
  $^{53}$ {\eightit Yale University, New Haven, Connecticut 06520  } \\
%\end{center}
}

